Adaptive Adversarial Attack on Scene Text Recognition

Recent studies have shown that state-of-the-art deep learning models are vulnerable to the inputs with small perturbations (adversarial examples). We observe two critical obstacles in adversarial examples: (i) Strong adversarial attacks (e.g., C&W attack) require manually tuning hyper-parameters and take a long time to construct an adversarial example, making it impractical to attack real-time systems; (ii) Most of the studies focus on non-sequential tasks, such as image classification, yet only a few consider sequential tasks. In this work, we speed up adversarial attacks, especially on sequential learning tasks. By leveraging the uncertainty of each task, we directly learn the adaptive multi-task weightings, without manually searching hyper-parameters. A unified architecture is developed and evaluated for both non-sequential tasks and sequential ones. To validate the effectiveness, we take the scene text recognition task as a case study. To our best knowledge, our proposed method is the first attempt to adversarial attack for scene text recognition. Adaptive Attack achieves over 99.9\% success rate with 3-6X speedup compared to state-of-the-art adversarial attacks.

==> back_adv.tex <==
Adversarial examples are imperceptible to humans but can easily fool deep neural networks in the testing/deploying stage. People have studied adversarial examples of machine learning models (machine learning evasion attacks) since 2012~\cite{biggio2017wild}. 
% Adversarial examples at the training stage (data poisoning) is another interesting topic, but we will not discuss it in the paper.

With rapid progress and great success in a wide spectrum of applications, deep learning is being applied in many safety-critical environments. 
The vulnerability to adversarial examples becomes one of the major obstacles for applying deep neural networks in many safety-critical scenarios. Most existing studies on adversarial examples focus on computer vision related tasks: image classification~\cite{szegedy2013intriguing}, face recognition~\cite{sharif2016accessorize}, reinforcement learning~\cite{huang2017adversarial}, and semantic segmentation~\cite{hendrik2017universal}. Only a few studies have been devoted to sequential domains, such as speech recognition~\cite{carlini2018audio} and reading comprehension~\cite{jia2017adversarial}. 

Iterative attacks have been prevalent in adversarial attacks due to high success rates and small perturbations: iteratively searching and updating the perturbations based on the gradient of the output of the victim model. In contrast, one-time attacks update the adversarial perturbations only once and they are usually used in real-time systems. For example, \cite{huang2017adversarial} and \cite{kos2017delving} leveraged a one-time attack, Fast Gradient Sign Method (FGSM)~\cite{goodfellow2014explaining}, to attack reinforcement learning systems due to the requirement of quick response to the real-time input. However, it is easy to detect/defend one-time attacks.

The magnitude of perturbations is measured by $\ell_p$ norm ($p=0,1,\infty$). A few studies use other measurements (\eg, SSIM~\cite{rozsa2016adversarial}, spatial transformation~\cite{engstrom2017rotation}). 
% \cite{sharif2018suitability} analyzed the suitability of these measurements. 
In this paper, we only consider $\ell_2$ norm, which can be comparable to most of the current work. 
For further details on adversarial attacks, we refer to~\cite{yuan2019adversarial}. 

To our best knowledge, we are the first group to successfully generate sequential adversarial examples on a scene text recognition task.

==> back_ctc.tex <==
Connectionist Temporal Classification (CTC)~\cite{graves2006connectionist} is designed for training sequence-to-sequence neural network on sequential classification tasks, where the alignment between the inputs and the target labels is unknown. 
% CTC aims at transforming the network outputs into a conditional probability distribution over label sequences and selects the most probable labeling for a given input sequence. 
% We briefly summarize the key details. More details can be found in~\cite{graves2006connectionist}.
We briefly introduce CTC in this section. We will later generate adversarial examples based on CTC algorithm.

Let $\mathcal{X}$ be the input domain, a single frame of input
and $\mathcal{Y}$ be the range, the (finite) alphabet $\mathcal{S}$ of labels plus a blank label.
For an input sequence of $T$ frames $x_t \in \mathcal{X}$, the network will output a probability distribution over the output domain for each frame, where we denote the mapping function as $\mathcal{F}$. Denote by $y^t_k$ the activation of output unit $k \in \mathcal{Y}$ at frame $t$ and $y^t_k$ is then interpreted as the
probability of observing label $k$ at frame $t$. We use $\pi$ to denote one path: a sequence of characters $y^t_{\pi_t}$, $\pi_t \in \mathcal{Y}$.

While $\mathcal{F}$ maps every frame to a probability distribution over the characters, this does not directly give us a probability distribution over all paths. 
To achieve this, we define a label $l$, which can be obtained by removing all blanks and repeated labels from the path $\pi$.
% (\eg, $\mathcal{B}(a-ab−) = \mathcal{B}(-aa--abb) = aab)$. 
Given an input sequence $X$, the probability of a given path $\pi$ can be written as:
\begin{equation}
  \Pr(\pi|x) = \prod_{t=1}^T y^t_{\pi_t}
\end{equation}
We define $\mathcal{B}$ as the conditional probability of a given labeling $l$. We then sum up the probabilities of all the paths:
\begin{equation}
\label{eq:ctc1}
  \Pr(l | x) = \sum_{\pi \in \mathcal{B}^{-1}(l)} \Pr(\pi| x)
\end{equation}
It is numerically stable to calculate the probability by negative log likelihood: $CTC_{Loss}(x, l) = - \log \Pr(l|x)$.
Given the above formulation, the output of the classifier should be the most probable labeling for the input sequence:
\begin{equation}
h(X) = \argmax_{l \in \mathcal{S}^{\leq T}} \Pr(l|x).
\end{equation}
% Greedy search is usually used to get the most probable path from the probability. 

Computing $h(x)$ requires searching an exponential space and usually to be approximated in two ways: greedy path decoding and beam search decoding. 
In our experiment, we use greedy path decoding for simplicity, which simultaneously evaluates the likelihood of multiple alignments $\pi$ and then chooses the most likely path under these alignments. 
% The first method (Greedy  Path Decoding) is based on the assumption that the most probable path will correspond to the most probable labeling:
% \begin{equation}
% \begin{aligned}
% h(x) & \approx  \mathcal{B}(\pi^*) \\
% where\; \pi^* & = \argmax_{\pi \in \mathcal{Y}^T} P(\pi|x)
% \end{aligned}
% \end{equation}

% The other method (Beam Search Decoding) simultaneously evaluates the likelihood of multiple alignments $\pi$ and then chooses the most likely path $\rho$ under these alignments. In our experiment, we use Greedy Path Decoding for simplicity.

==> back_scene.tex <==
Scene text recognition tasks aim at decoding a sequence of text characters from a cropped but variable-length word image. 
Before the use of neural networks, previous studies focus on developing individual character classifiers, following the pipeline of conventional OCR techniques: a character-level segmentation, then an isolated character classifier and post-processing for final recognition. However, their performance was severely limited by the character segmentation. More importantly, recognizing individual character with finite-length context sliding windows discards meaningful context information between characters, reducing the model's reliability and robustness.

% Apart from character-level approaches, 
Recent scene text recognition approaches focus on mapping the entire image to a word string, either with hand-crafted features or deep learning features. \cite{almazan2014word} proposed a subspace regression method to jointly embed both word images and their text strings into a common
subspace, resulting in solving a nearest neighbor problem. \cite{jaderberg2014synthetic} developed a CNN model to cast the word recognition into a multi-class classification problem. They further proposed a CNN based architecture, incorporating a conditional random field graphical model for unconstrained text recognition~\cite{jaderberg2014deep}. \cite{su2014accurate} built an RNN with HOG features and casted text recognition as a sequence labeling problem. \cite{he2016reading} and \cite{shi2017end} extracted rich visual features from a CNN; then a sequence labeling is carried out with LSTM and CTC. 
\cite{lee2016recursive} incorporated attention modeling into recursive recurrent neural networks for lexicon-free optical character recognition in natural scene images. \cite{shi2016robust} and \cite{BMVC2016_43} extended the work of~\cite{jaderberg2015spatial} to transform a distorted text region into a canonical pose suitable for recognition. In our experiment, we train a similar recognition model, based on the state-of-the-art approach, Convolutional Recurrent Neural Network (CRNN)~\cite{shi2017end}.

